Power Systems Performance under 5G Radio Access Network in a Co-Simulation Environment

Communication can improve control of important system parameters by allowing different grid components to communicate their states with each other. This information exchange requires a reliable and fast communication infrastructure. 5G communication can be a viable means to achieve this objective. This paper investigates the performance of several smart grid applications under a 5G radio access network. Different scenarios including set point changes and transients are evaluated, and the results indicate that the system maintains stability when a 5Gnetwork is used to communicate system states.

==> results.tex <==
\section{Results}
\label{section - Results}

\begin{itemize}
    \item List the general benefit of Age based scheduling in terms of increased PDR, throughput and safety.
    \item Compare AoI and TA-AoII. Point out the reduction in rates while not compromising on the safety performance.
\end{itemize}
